Two-Loop SL(2) Form Factors and Maximal Transcendentality

Form factors of composite operators in the SL(2) sector of N=4 SYM theory are studied up to two loops via the on-shell unitarity method. The non-compactness of this subsector implies the novel feature and technical challenge of an unlimited number of loop momenta in the integrand's numerator. At one loop, we derive the full minimal form factor to all orders in the dimensional regularisation parameter. At two loops, we construct the complete integrand for composite operators with an arbitrary number of covariant derivatives, and we obtain the remainder functions as well as the dilatation operator for composite operators with up to three covariant derivatives. The remainder functions reveal curious patterns suggesting a hidden maximal uniform transcendentality for the full form factor. Finally, we speculate about an extension of these patterns to QCD.

==> picturemacro.tex <==
\makeatletter

%% Form factor diagrams
% xkeyval definitions
\define@boolkey{FDff}{oneloop}[true]{}
\define@boolkey{FDff}{twoloop}[true]{}
% \define@boolkey{FDff}{black}[true]{}
% \define@boolkey{FDff}{blue}[true]{}
% \define@boolkey{FDff}{green}[true]{}
\define@boolkey{FDff}{reflected}[true]{}
\define@boolkey{FDff}{fancy}[true]{}
% \define@boolkey{FDff}{small}[true]{}
% \define@key{FDff}{loops}%
%  {\def\FDffloops{#1}}%
\define@key{FDff}{legs}%
 {\def\FDfflegs{#1}}%
\define@key{FDff}{scaled}%
 {\def\FDffscaled{#1}}%
\presetkeys{FDff}{%
% loops=0,%
scaled=1,
legs=2,%
reflected=false,%
fancy=false,%
oneloop=false,%
twoloop=false%
% red=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDff[1][]{%
 \setkeys{FDff}{#1}%
% 
\setlength{\unitlength}{\FDffscaled mm}%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,1)(1,1){%
\scalebox{1}{%
\fmfstraight%
\begin{fmfchar*}(25,14)%
\expandafter\fmfcmd{%
dash_len := 0.5; 
newinternal numeric loops,legs,scald;
legs:=\FDfflegs;
scald:=\FDffscaled;
% loops:=\FDffloops;
}%
% \begin{fmfshrink}{1}
% outgoing
\ifKV@FDff@reflected
\fmfright{vq}
\fmfleftn{vp}{\FDfflegs}
\else
\fmfleft{vq}
\fmfrightn{vp}{\FDfflegs}
\fi
% internal lines left
\fmf{dbl_plain,tension=legs}{vq,v1}
% internal lines right
\ifKV@FDff@fancy
\fmf{plain}{v1,vp1}
\begin{fmffor}{n}{2}{1}{\FDfflegs-2}
\fmf{phantom}{v1,vp[n]}
\end{fmffor}
\begin{fmffor}{n}{\FDfflegs-1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\else
\begin{fmffor}{n}{1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\fi
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone; vertone = vloc(__v1); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
%  \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
%  \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
%  \ifKV@FDff@spacetime
%  \fmfiv{label=$\scriptstyle q$}{vertq}
%  \fmfiv{label=$\scriptstyle p_1$}{vertpone}
%  \fmfiv{label=$\scriptstyle p_2$}{vertptwo}
% \else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
% \ifKV@FDff@flavour
%  \fmfiv{label=$\scriptstyle K$}{verttwo+(26,14)}
%  \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
%  \fmfiv{label=$\scriptstyle L$}{verttwo+(26,-14)}
%  \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
% \else\fi
% 
% BLOB
  \fmfiv{decor.shape=circle,decor.filled=60,decor.size=30*scald}{vertone}
\ifKV@FDff@fancy
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=30*scald,label=$\ncsusyF_n$,l.d=0}{vertone}
  \ifKV@FDff@reflected
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=180}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=190}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=200}{vertone}
  \else
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=0}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-10}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-20}{vertone}
  \fi
\else\fi  
\ifKV@FDff@oneloop
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=15*scald}{vertone}
\else\fi
\ifKV@FDff@twoloop
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor black;}
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor black;}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(7,0)}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(-7,0)}
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
\fmfcurved
}}}%
}




%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDinline}{cutlabels}[true]{}
\define@boolkey{FDinline}{bubble}[true]{}
\define@boolkey{FDinline}{bubblethree}[true]{}
\define@boolkey{FDinline}{bubbletwoone}[true]{}
\define@boolkey{FDinline}{bubbletwoonerev}[true]{}
\define@boolkey{FDinline}{triangle}[true]{}
\define@boolkey{FDinline}{triangletwoone}[true]{}
\define@boolkey{FDinline}{triangletwoonerev}[true]{}
\define@boolkey{FDinline}{trianglethreetop}[true]{}
\define@boolkey{FDinline}{trianglethreebot}[true]{}
\define@boolkey{FDinline}{box}[true]{}
\define@boolkey{FDinline}{rainbow}[true]{}
\define@boolkey{FDinline}{fliprainbow}[true]{}
\define@boolkey{FDinline}{rainbownonplanar}[true]{}
\define@boolkey{FDinline}{fliprainbownonplanar}[true]{}
\define@boolkey{FDinline}{wedgetop}[true]{}
\define@boolkey{FDinline}{wedgebottom}[true]{}
\define@boolkey{FDinline}{wedgestartop}[true]{}
\define@boolkey{FDinline}{wedgestarbottom}[true]{}
\define@boolkey{FDinline}{itwo}[true]{}
\define@boolkey{FDinline}{fishtop}[true]{}
\define@boolkey{FDinline}{fishbottom}[true]{}
\define@boolkey{FDinline}{fishtopback}[true]{}
\define@boolkey{FDinline}{fishbottomback}[true]{}
\define@boolkey{FDinline}{trianglebubblethree}[true]{}
\define@boolkey{FDinline}{bubbletrianglethree}[true]{}
\define@boolkey{FDinline}{trianglesubbubbletop}[true]{}
\define@boolkey{FDinline}{trianglesubbubblebottom}[true]{}
\define@boolkey{FDinline}{trianglefishtop}[true]{}
\define@boolkey{FDinline}{trianglefishbottom}[true]{}
\define@boolkey{FDinline}{trianglefishtopback}[true]{}
\define@boolkey{FDinline}{trianglefishbottomback}[true]{}
\define@boolkey{FDinline}{trianglebridgebubbletop}[true]{}
\define@boolkey{FDinline}{trianglebridgebubblebottom}[true]{}
\define@boolkey{FDinline}{bubblevertical}[true]{}
\define@boolkey{FDinline}{sunrise}[true]{}
\define@boolkey{FDinline}{sunrisethree}[true]{}
\define@boolkey{FDinline}{bubbletriangle}[true]{}
\define@boolkey{FDinline}{doubletrianglethree}[true]{}
\define@boolkey{FDinline}{doubletriangletwo}[true]{}
\define@boolkey{FDinline}{doublebubble}[true]{}
\define@boolkey{FDinline}{boxtriangle}[true]{}
\define@boolkey{FDinline}{trianglebox}[true]{}
\define@boolkey{FDinline}{boxbubble}[true]{}
\define@boolkey{FDinline}{bubblebox}[true]{}
\define@boolkey{FDinline}{shiftedtriangletriangle}[true]{}
\define@boolkey{FDinline}{triangleshiftedtriangle}[true]{}
\define@boolkey{FDinline}{shiftedtrianglebubble}[true]{}
\define@boolkey{FDinline}{bubbleshiftedtriangle}[true]{}
\define@boolkey{FDinline}{masstop}[true]{}
\define@boolkey{FDinline}{massbottom}[true]{}
\define@boolkey{FDinline}{twomomenta}[true]{}
\define@boolkey{FDinline}{dermomenta}[true]{}
\define@boolkey{FDinline}{momentum}[true]{}
\define@boolkey{FDinline}{momentumarrow}[true]{}
\define@boolkey{FDinline}{altmomentum}[true]{}
\define@boolkey{FDinline}{twolabels}[true]{}
\define@boolkey{FDinline}{threelabels}[true]{}
\define@boolkey{FDinline}{cut}[true]{}
\define@boolkey{FDinline}{big}[true]{}
\define@boolkey{FDinline}{botdoublecut}[true]{}
\define@boolkey{FDinline}{topdoublecut}[true]{}
\define@boolkey{FDinline}{doublecut}[true]{}
\define@boolkey{FDinline}{slashdoublecut}[true]{}
\define@boolkey{FDinline}{bslashdoublecut}[true]{}
\define@boolkey{FDinline}{triplecut}[true]{}
\define@boolkey{FDinline}{alttriplecut}[true]{}
\define@boolkey{FDinline}{quadruplecut}[true]{}
\define@boolkey{FDinline}{splitlabels}[true]{}
\define@key{FDinline}{labelone}%
{\def\FDinlinelabelone{#1}}%
\define@key{FDinline}{labeltwo}%
{\def\FDinlinelabeltwo{#1}}%
\define@key{FDinline}{labelthree}%
{\def\FDinlinelabelthree{#1}}%
\define@key{FDinline}{toplabel}%
{\def\FDinlinetoplabel{#1}}%
\presetkeys{FDinline}{%
cutlabels=false,%
big=false,%
bubble=false,%
bubblethree=false,%
bubbletwoone=false,%
bubbletwoonerev=false,%
triangle=false,%
trianglethreetop=false,%
trianglethreebot=false,%
triangletwoone=false,%
triangletwoonerev=false,%
triangleshiftedtriangle=false,%
shiftedtriangletriangle=false,%
bubbleshiftedtriangle=false,%
shiftedtrianglebubble=false,%
box=false,%
rainbow=false,%
fliprainbow=false,%
rainbownonplanar=false,%
fliprainbownonplanar=false,%
wedgetop=false,%
wedgebottom=false,%
wedgestartop=false,%
wedgestarbottom=false,%
itwo=false,%
fishtop=false,%
fishbottom=false,%
fishtopback=false,%
fishbottomback=false,%
trianglesubbubbletop=false,%
trianglesubbubblebottom=false,%
trianglebridgebubbletop=false,%
trianglebridgebubblebottom=false,%
trianglefishtop=false,%
trianglefishbottom=false,%
trianglefishtopback=false,%
trianglefishbottomback=false,%
bubblevertical=false,%
sunrise=false,%
sunrisethree=false,%
massbottom=false,%
masstop=false,%
bubbletriangle=false,%
bubbletrianglethree=false,%
trianglebubblethree=false,%
bubblebox=false,%
boxbubble=false,%
trianglebox=false,%
boxtriangle=false,%
doubletriangletwo=false,%
doubletrianglethree=false,%
doublebubble=false,%
twomomenta=false,%
momentum=false,%
dermomenta=false,%
momentumarrow=false,%
altmomentum=false,%
twolabels=false,%
threelabels=false,%
cut=false,%
botdoublecut=false,%
topdoublecut=false,%
doublecut=false,%
slashdoublecut=false,%
bslashdoublecut=false,%
triplecut=false,%
alttriplecut=false,%
quadruplecut=false,%
splitlabels=false,%
toplabel=$\phantom{0}$,%
labelone=\phantom{0},%
labeltwo=\phantom{0},%
labelthree=\phantom{0}%
}{}
% Makro / FeynMP definitions
%straight galeries
\fmfstraight
\newcommand*\FDinline[1][]{%
 \setkeys{FDinline}{#1}%
% 
% BIG
\ifKV@FDinline@big
\unitlength=1mm
\else
\unitlength=0.666mm
\fi
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelone}}}
 \else\fi
 \else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelthree}}}
 \else\fi
 \else\fi
%%% diagrams
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-11\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(2,3)(2,3){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.5mm; 
}%
% \begin{fmfshrink}{0.5}
\fmfstraight
% cut
\ifKV@FDinline@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% BOX
\ifKV@FDinline@box
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0}{v1,v2}
\fmf{plain,right=0}{v1,v3}
% internal lines right
\fmf{plain,tension=0.8}{v2,vp1}
\fmf{plain,tension=0.8}{v3,vp3}
% top and bottom
% \fmf{phantom,tension=1.8}{v2,vt}
% \fmf{phantom,tension=1.8}{v3,vb}
% right corner
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% slash double cut
\ifKV@FDinline@slashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v2,v4}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v2,v4}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% back slash double cut
\ifKV@FDinline@bslashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v3,v4}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v3,v4}
\else\fi
\else\fi
\fmffreeze
\fmf{plain,left=0}{v2,v4}
\fmf{plain,right=0}{v3,v4}
\fmf{plain,tension=5}{v4,vp2}
\else\fi
% BUBBLE
\ifKV@FDinline@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
\else\fi
% BUBBLETHREE
\ifKV@FDinline@bubblethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
% two momenta
\ifKV@FDinline@twomomenta
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l_1$}{v2,v1}
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l_2$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% BUBBLETWOONE
\ifKV@FDinline@bubbletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLETWOONEREV
\ifKV@FDinline@bubbletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLE VERTICAL
\ifKV@FDinline@bubblevertical
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{point length(p1)/2 of p1
-- point length(p2)/2 of p2}
\else\fi
% FISHTOP
\ifKV@FDinline@fishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom_smallcut}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom_smallcut}{subpath (length(p2),0*length(p2)) of p2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0*length(p2)) of p2}
\else\fi
\else\fi
% FISHBOTTOMBACK
\ifKV@FDinline@fishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 0}(point length(p1) of p1)}
\else\fi
% FISHTOPBACK
\ifKV@FDinline@fishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 0}(point 0length(p2) of p2)}
\else\fi
% FISHBOTTOM
\ifKV@FDinline@fishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,right=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom_smallcut}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom_smallcut}{subpath (length(p1),0*length(p1)) of p1}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (length(p1),0*length(p1)) of p1}
\else\fi
\else\fi
% SUNRISE
\ifKV@FDinline@sunrise
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel,tension=0.5}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,right=0,tension=0}{v1,v2}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% SUNRISETHREE
\ifKV@FDinline@sunrisethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tension=0.5,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% DOUBLEBUBBLE
\ifKV@FDinline@doublebubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle right
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v2,v3}
\fmf{plain,right=0.7}{v2,v3}
% internal lines right
\fmf{plain,tension=1.5}{v3,vp1}
\fmf{plain,tension=1.5}{v3,vp2}
\else\fi
% BUBBLETRIANGLE
\ifKV@FDinline@bubbletriangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2,v2t}
\fmf{plain,right=0.0}{v2,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLE
\ifKV@FDinline@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l_1$,l.d=2.5,label.side=left}{v1,v2t}
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% TRIANGLEBRIDGEBUBBLETOP
\ifKV@FDinline@trianglebridgebubbletop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmffreeze
% middle
\fmf{plain,tension=3}{vm,v2b}
\fmf{plain,tension=1,left=0.5}{vm,v2t}
\fmf{plain,tension=1,right=0.5}{vm,v2t}
\else\fi
% TRIANGLEBRIDGEBUBBLEBOTTOM
\ifKV@FDinline@trianglebridgebubblebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmffreeze
% middle
\fmf{plain,tension=3}{vm,v2t}
\fmf{plain,tension=1,left=0.5}{vm,v2b}
\fmf{plain,tension=1,right=0.5}{vm,v2b}
\else\fi
% TRIANGLETWOONE
\ifKV@FDinline@triangletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETWOONEREV
\ifKV@FDinline@triangletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETHREETOP
\ifKV@FDinline@trianglethreetop
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=2.5,label.side=right}{v2t,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=2.5,label.side=left}{v2b,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2t,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
\else\fi
% TRIANGLETHREEBOT
\ifKV@FDinline@trianglethreebot
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=2.5}{v2b,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=right,l.d=2.5}{v2t,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2b,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
\else\fi
% DOUBLETRIANGLETHREE
\ifKV@FDinline@doubletrianglethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2b,vp3}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
\else\fi
% BUBBLETRIANGLETHREE
\ifKV@FDinline@bubbletrianglethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
% \fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\fmf{phantom,tension=2}{v2t,vp1}
\fmf{plain,tension=0}{v2m,vp1}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2b,vp3}
\else\fi
% TRIANGLEBUBBLETHREE
\ifKV@FDinline@trianglebubblethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{phantom,left=0.0}{v1,v2b}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2t}
% \fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2t}
% internal lines right
\fmf{phantom,tension=2}{v2b,vp3}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2t,vp1}
\else\fi
% DOUBLETRIANGLETWO
\ifKV@FDinline@doubletriangletwo
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp3}
\else
\fmf{plain,tension=2}{v2b,vp3}
\fi
\fmf{phantom,tension=2}{v2m,vp2}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
\else\fi
% ITWO
\ifKV@FDinline@itwo
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0,right=0.5}{v2t,v2b}
\fmf{plain,tension=0,left=0.5}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% RAINBOW
\ifKV@FDinline@rainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,label.side=left,l.d=2.5}{v1,v2t}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% \fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% \fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% FLIPPED RAINBOW
\ifKV@FDinline@fliprainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{phantom,left=0.0,tension=0.8}{vq,v2t}
\fmf{phantom,right=0.0,tension=0.8}{vq,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle left
\fmf{phantom,left=0.0,tension=0.0001,tag=1}{v1,v3t}
\fmf{phantom,right=0.0,tension=0.0001}{v1,v3b}
\fmf{plain,left=0.0,tension=0.00005}{v1,v2t}
\fmf{plain,right=0.0,tension=0.00005}{v1,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=2.5}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0,tag=1}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.8}{v3t,vp1}
\fmf{plain,tension=1.8}{v3b,vp2}
% double line
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v3t)}
\fmfiset{p2}{vpath1(__v3t,__v3b)}
% \fmfi{double}{point 0*length(p1)/2 of p1 -- point length(p2)/2 of p2}
\fmfi{double}{point 0*length(p1)/2 of p1 -- 0.5*((point length(p2)/2 of p2)+(point 0*length(p1)/2 of p1))}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% BOXTRIANGLE
\fmfstraight
\ifKV@FDinline@boxtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3t,v3m}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v3t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% TRIANGLEBOX
\fmfstraight
\ifKV@FDinline@trianglebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2t,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=left,l.d=2.5}{v2m,v3m}
\else\fi
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v3b}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% WEDGETOP
\ifKV@FDinline@wedgetop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v2t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% WEDGESTARTOP
\ifKV@FDinline@wedgestartop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines middle right
\fmf{plain,right=0.0}{v2b,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
% middle
\fmffreeze
\fmf{plain,tension=1}{v2t,vm}
\fmf{plain,tension=0}{vm,v2b}
\fmf{plain,tension=1}{vm,v3b}
\else\fi
% WEDGEBOTTOM
\ifKV@FDinline@wedgebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% WEDGESTARBOTTOM
\ifKV@FDinline@wedgestarbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
% middle
\fmffreeze
\fmf{plain,tension=1}{v2b,vm}
\fmf{plain,tension=0}{vm,v2t}
\fmf{plain,tension=1}{vm,v3t}
\else\fi
% RAINBOW NONPLANAR
\ifKV@FDinline@rainbownonplanar
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0,rubout}{v2t,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% FLIPPED RAINBOW NONPLANAR
\ifKV@FDinline@fliprainbownonplanar
% outgoing
\fmfleft{vp1}
\fmfright{vp2}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{plain,tension=5}{vp1,vl}
% internal lines middle
\fmf{phantom,tension=10}{vt,vta}
\fmf{plain,tension=1}{vta,v1}
\fmf{plain,tension=1}{vba,v1}
\fmf{phantom,tension=10}{vba,vb}
% internal lines middle left
\fmf{plain,tension=1}{vta,vl}
\fmf{plain,tension=1}{vba,vl}
% internal lines middle right
\fmf{plain,tension=1}{vta,vr}
\fmf{plain,tension=1}{vba,vr}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5,label.side=right}{v1,vta}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{vta,v1}
\else\fi
% internal lines right
\fmf{plain,tension=5}{vr,vp2}
% double line
\fmf{phantom,tension=0,tag=1}{vl,v1}
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__vl,__v1)}
\fmfi{double}{subpath (length(p1),0.6*length(p1)) of p1}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{vr,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vl,vba}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=right,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{vr,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{vl,vba}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vl}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,left=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{vr,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=left,right=0,tension=0}{vl,vta}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
\fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
% \fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% \fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v1,vba}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
\else\fi
% TRIANGLEFISHTOP
\ifKV@FDinline@trianglefishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p1)/3 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmfi{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{(point length(p2) of p2)..(point 2length(p1)/3 of p1)}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
\else\fi
% % TRIANGLEFISHBOTTOMBACK
\ifKV@FDinline@trianglefishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p2)/3 of p2){dir 30}..{dir -70}(point 0length(p2) of p2)}
\else\fi
% TRIANGLEFISHTOPBACK
\ifKV@FDinline@trianglefishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p1)/3 of p1){dir -30}..{dir 70}(point length(p1) of p1)}
\else\fi
% TRIANGLEFISHBOTTOM
\ifKV@FDinline@trianglefishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p2)/3 of p2){dir 90}..{dir 180}(point length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmfi{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{(point length(p2) of p2)..(point 1length(p2)/3 of p2)}
\else\fi
\else\fi
% TRIANGLESUBBUBBLEBOTTOM
\ifKV@FDinline@trianglesubbubblebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point length(p2) of p2){dir 0}..{dir -70}(point 0length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
\else\fi
% TRIANGLESUBBUBBLETOP
\ifKV@FDinline@trianglesubbubbletop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 0length(p1) of p1){dir 0}..{dir 70}(point length(p1) of p1)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_1$,l.s=left,l.d=2.5}{v1,v2t}
\fmf{electron,tension=0,left=0,label=$\scriptstyle l_3$,l.s=right,l.d=2.5}{v1,v2b}
\else\fi
\else\fi
% BOXBUBBLE
\fmfstraight
\ifKV@FDinline@boxbubble
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3m}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% BUBBLEBOX
\fmfstraight
\ifKV@FDinline@bubblebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v2m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% SHIFTEDTRIANGLETRIANGLE
\fmfstraight
\ifKV@FDinline@shiftedtriangletriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% SHIFTEDTRIANGLEBUBBLE
\fmfstraight
\ifKV@FDinline@shiftedtrianglebubble
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v3m}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
% \fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v3m}
\fmf{phantom_smallcut,right=0.0,tension=0}{v1,v2m}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2m}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,left=0.7,tension=0,l.d=8}{v1,v3m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,right=0.0,tension=0,l.s=left,l.d=13}{v1,v2m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.7,tension=0,l.d=8}{v1,v2m}
\else\fi
\else\fi
% alttriple cut
\ifKV@FDinline@alttriplecut
% \fmf{phantom_smallcut,left=0.7,tension=0}{v1,v3m}
\fmf{phantom_hugecut,right=0.0,tension=0}{v1,v2m}
% \fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2m}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,left=0.7,tension=0,l.d=4,l.s=right}{v1,v3m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,right=0.0,tension=0,l.s=left,l.d=18}{v1,v2m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.0,tension=0,l.d=18}{v1,v2m}
\else\fi
\else\fi
\else\fi
% BUBBLESHIFTEDTRIANGLE
\fmfstraight
\ifKV@FDinline@bubbleshiftedtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
% \fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v2m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v3m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2m}
\fmf{phantom_smallcut,right=0.0,tension=0}{v1,v2m}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v3m}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,left=0.7,tension=0,l.d=8}{v1,v2m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,right=0.0,tension=0,l.s=right,l.d=13}{v1,v2m}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.7,tension=0,l.d=8}{v1,v3m}
\else\fi
\else\fi
\else\fi
% TRIANGLESHIFTEDTRIANGLE
\fmfstraight
\ifKV@FDinline@triangleshiftedtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,right=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2t}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v2m,v2t}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5,l.s=left}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp3}
\fmf{plain,tension=2}{v3t,vp1}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% LABELS
%
% THREE LABELS  
 \ifKV@FDinline@threelabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % labels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=180,l.d=4}{vertpthree}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=0,l.d=4}{vertpthree}
 \fi
 \else\fi
%
% TWO LABELS  
 \ifKV@FDinline@twolabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % labels
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=180,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \fi
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
% Set back to curved galeries
 \fmfcurved
}}}%
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\fi\else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabelthree}}}}
 \fi\else\fi
}


%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDdimred}{zigzagbubble}[true]{}
\define@boolkey{FDdimred}{scalarbubble}[true]{}
\define@boolkey{FDdimred}{gluonbubble}[true]{}
\define@boolkey{FDdimred}{zigzagfermion}[true]{}
\define@boolkey{FDdimred}{scalarfermion}[true]{}
\define@boolkey{FDdimred}{gluonfermion}[true]{}
\define@boolkey{FDdimred}{bubble}[true]{}
\define@boolkey{FDdimred}{triangle}[true]{}
\define@boolkey{FDdimred}{cut}[true]{}
\define@key{FDdimred}{toplabel}%
{\def\FDdimredtoplabel{#1}}%
\define@key{FDdimred}{topleglabel}%
{\def\FDdimredtopleglabel{#1}}%
\define@key{FDdimred}{bottomleglabel}%
{\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDdimred}{%
zigzagbubble=false,%
scalarbubble=false,%
gluonbubble=false,%
zigzagfermion=false,%
scalarfermion=false,%
gluonfermion=false,%
bubble=false,%
triangle=false,%
cut=false,%
toplabel=$\phantom{0}$,%
topleglabel=$\phantom{0}$,%
bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDdimred[1][]{%
 \setkeys{FDdimred}{#1}%
% 
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{0.5}
% cut
\ifKV@FDdimred@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% SCALARBUBBLE
\ifKV@FDdimred@scalarbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONBUBBLE
\ifKV@FDdimred@gluonbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{wiggly,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{wiggly,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGBUBBLE
\ifKV@FDdimred@zigzagbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{zigzag,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{zigzag,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% BUBBLE
\ifKV@FDdimred@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.2}{v2,vp1}
\fmf{plain,tension=1.2}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% TRIANGLE
\ifKV@FDdimred@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDdimredtoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.2}{v2t,vp1}
\fmf{plain,tension=1.2}{v2b,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGFERMION
\ifKV@FDdimred@zigzagfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{zigzag,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% SCALARFERMION
\ifKV@FDdimred@scalarfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONFERMION
\ifKV@FDdimred@gluonfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{photon,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}


%% flow diagrams
% xkeyval definitions
\define@boolkey{FDflow}{spacetime}[true]{}
\define@boolkey{FDflow}{flavour}[true]{}
\define@boolkey{FDflow}{black}[true]{}
\define@boolkey{FDflow}{blue}[true]{}
\define@boolkey{FDflow}{green}[true]{}
\define@boolkey{FDflow}{red}[true]{}
\define@boolkey{FDflow}{fermion}[true]{}
\define@boolkey{FDflow}{twopoint}[true]{}
\define@boolkey{FDflow}{cutleft}[true]{}
\define@boolkey{FDflow}{cutright}[true]{}
\define@boolkey{FDflow}{cutmiddle}[true]{}
% \define@key{FDdimred}{bottomleglabel}%
% {\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDflow}{%
flavour=false,%
spacetime=false,%
black=false,%
blue=false,%
green=false,%
red=false,%
fermion=false,%
twopoint=false,%
cutmiddle=false,%
cutright=false,%
cutleft=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDflow[1][]{%
 \setkeys{FDflow}{#1}%
%
\fmfstraight
%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-10\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(0,3)(4,3){%
\scalebox{1}{%
\begin{fmfchar*}(25,14)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{1}
% FERMIONS
\ifKV@FDflow@fermion
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp3}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertpthree, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir -180}..{dir 0}(verttwo+(20,0))}
 \fmfi{plain}{(vertpthree){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
% TWO-POINT FUNCTION
 \else
 \ifKV@FDflow@twopoint
 % outgoing
\fmfleft{vq1}
\fmfright{vq2}
% internal lines left
\fmf{dbl_plain,tension=10}{vq1,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
\fmf{phantom,left=1.0}{v2,v3}
\fmf{phantom,right=1.0}{v2,v3}
% internal lines right
\fmf{dbl_plain,tension=10}{v3,vq2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertqone,  vertqtwo, vertone, verttwo, vertthree; vertqone = vloc(__vq1); vertone = vloc(__v1);verttwo = vloc(__v2);vertthree = vloc(__v3); vertqtwo = vloc(__vq2); }
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir 120}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir -120}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % SCALARS 
 \else
 % outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fi
 \fi
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
 \ifKV@FDflow@spacetime
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle q$}{vertqone}
 \fmfiv{label=$\scriptstyle q$}{vertqtwo}
 \else
 \fmfiv{label=$\scriptstyle q$}{vertq}
 \fmfiv{l.a=0,label=$\scriptstyle p_1$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle p_2$}{vertptwo}
 \ifKV@FDflow@fermion
 \fmfiv{label=$\scriptstyle p_3$}{vertpthree}
\else\fi
\fi
\else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
\ifKV@FDflow@flavour
 \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
 \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
 \ifKV@FDflow@fermion 
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle A$}{vertptwo}
 \fmfiv{l.a=0,label=$\scriptstyle B$}{vertpthree}
 \else
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle K$}{verttwo+(+16,14)}
 \fmfiv{label=$\scriptstyle L$}{verttwo+(+16,-14)}
 \else
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle L$}{vertptwo}
 \fi
 \fi
\else\fi
% 
\ifKV@FDflow@black
 \fmfiv{decor.shape=circle,decor.filled=60,decor.size=40}{verttwo}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,-7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,-7)}
\else\fi
% 
\ifKV@FDflow@blue
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=blue}{(verttwo+(0,-8)){dir 90}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@red
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=red}{(verttwo+(11,0)){dir 180}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=red}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -135}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=red}{(verttwo+(20/sqrt(2),20/sqrt(2))){dir -135}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@green
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=green}{(verttwo+(10/sqrt(2),-10/sqrt(2))){dir +45}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir 45}(verttwo-(2/sqrt(2),2/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(2/sqrt(2),2/sqrt(2))){dir 45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
\else\fi
\fmftop{vt}
\fmfbottom{vb}
\fmfposition
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair verttop, vertbot; verttop = vloc(__vt); vertbot = vloc(__vb); }
\ifKV@FDflow@cutmiddle
\fmfi{dashes}{(verttop+(0,8))--(vertbot+(0,-8))}
\else\fi
\ifKV@FDflow@cutleft
\fmfi{dashes}{(verttop+(-11,8))--(vertbot+(-11,-8))}
\else\fi
\ifKV@FDflow@cutright
\fmfi{dashes}{(verttop+(11,8))--(vertbot+(11,-8))}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}











\makeatother

\newcommand{\initialisepictures}{
\fmfcmd{%
thin := 1pt; % dimension of the lines
thick := 2thin;
arrow_len := 3mm;
arrow_ang := 15;
curly_len := 3mm;
dash_len :=0.5; % 'photon' lines
% dash_space := 4mm;
dot_len := 0.75mm; % 'photon' lines
wiggly_len := 2mm; % 'photon' lines
wiggly_slope := 60;
zigzag_len := 2mm;
zigzag_width := 2thick;
decor_size := 5mm;
dot_size := 2thick;
}
\fmfcmd{%
hugemarksize=10mm;
%
def draw_hugecut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =hugemarksize*unitvector direction t of p;
    dma =hugemarksize*unitvector direction t of p rotated -90;
    dmb =hugemarksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 2bp off 2bp on 2bp) withcolor black);
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_hugecut expr p =
    save amid;
    amid=.5*arclength p;
    draw_hugecut(p, amid);
    draw p;
enddef;
}
\fmfcmd{%
marksize=7mm;
%
def draw_cut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =marksize*unitvector direction t of p;
    dma =marksize*unitvector direction t of p rotated -90;
    dmb =marksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 6bp off 12bp on 6bp));
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_cut expr p =
    save amid;
    amid=.5*arclength p;
    draw_cut(p, amid);
    draw p;
enddef;
}
\fmfcmd{%
smallmarksize=4mm;
%
def draw_smallcut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =smallmarksize*unitvector direction t of p;
    dma =smallmarksize*unitvector direction t of p rotated -90;
    dmb =smallmarksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 2bp off 2bp on 2bp) withcolor black);
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_smallcut expr p =
    save amid;
    amid=.5*arclength p;
    draw_smallcut(p, amid);
    draw p;
enddef;
}
}
